Efficient Distributed Quantum Computing

We provide algorithms for efficiently addressing quantum memory in parallel. These imply that the standard circuit model can be simulated with low overhead by the more realistic model of a distributed quantum computer. As a result, the circuit model can be used by algorithm designers without worrying whether the underlying architecture supports the connectivity of the circuit. In addition, we apply our results to existing memory intensive quantum algorithms. We present a parallel quantum search algorithm and improve the time-space trade-off for the Element Distinctness and Collision problems.

==> models_tikz.tex <==
\begin{minipage}[b]{0.5\linewidth}
\center
\begin{tikzpicture}[rounded corners,scale=0.75]
\path[use as bounding box] (0,-2) rectangle (7,4);
%\shade[ball color=blue] (3.5,4) circle (0.25cm);
%\draw[color=blue, style=dashed] (3.5,4) circle (0.5cm);
\shade[ball color=blue] (3.5,4) circle (0.5cm);
\foreach \x in {0,1,2,3}
  \draw (2*\x ,0) rectangle +(1,1);

\foreach \x in {0,1,2,3}
  \draw (3.5,4) -- (2*\x+0.5,1);
  
\shade[ball color=blue] (3.5,4) circle (0.5cm);

\node at (3.5,5) {(a)};
\end{tikzpicture}


\begin{tikzpicture}[rounded corners,scale=0.75]
\path[use as bounding box] (0,0) rectangle (7,5);

\foreach \x in {0,1,2,3}
  \draw (2*\x ,0) rectangle +(1,1);

\foreach \x in {0,1,2,3}
  \foreach \y in {0,1,2,3}
    \draw (2*\y+0.5,4) -- (2*\x+0.5,1);

\foreach \x in {0,1,2,3}
  \shade[ball color=blue] (2*\x+0.5,4) circle (0.25cm);

\node at (3.5,5.5) {(b)};
\end{tikzpicture}

\end{minipage}
\hspace{0.5cm}
\begin{minipage}[b]{0.5\linewidth}
\center
\begin{tikzpicture}[rounded corners,scale=0.75]
\path[use as bounding box] (0,-1.5) rectangle (8,5);

\foreach \x in {0,1,2,3}
  \draw (2*\x ,0) rectangle +(1,1);

\foreach \x in {0,1,2,3}
  \foreach \y in {0,1}
    \pgfmathparse{2*mod(\y+\x,4) + 0.5}
    \draw (\pgfmathresult,4) -- (2*\x+0.5,1);

\foreach \x in {0,1,2,3}
  \shade[ball color=blue] (2*\x+0.5,4) circle (0.25cm);

\node at (3.5,5) {(c)};
\end{tikzpicture}

\begin{tikzpicture}[rounded corners,scale=0.75]
\path[use as bounding box] (-3,-1) rectangle (5,4.6);

\foreach \x in {0,1}
  \foreach \y in {0,1}
  \draw (4.5*\x-2,4.5*\y-2) rectangle +(1,1);

\foreach \x in {0,1}
  \foreach \y in {0,1}
  \draw (3.5*\x-1,3.5*\y-1) -- (1.5*\x,1.5*\y);

\draw (0,0) .. controls (-1,0.75) .. (-1.5,2.5);
\draw (1.5,0) .. controls (0.75,-1) .. (-1,-1.5);
\draw (1.5,1.5) .. controls (2.5,0.75) .. (3,-1);
\draw (0,1.5) .. controls (0.75,2.5) .. (2.5,3);

\draw[style=dashed] (0.5,0.5) rectangle +(-3.0,-2.75);
\draw[style=dashed] (1,0.5) rectangle +(3.0,-2.75);
\draw[style=dashed] (0.5,1) rectangle +(-3.0,2.75);
\draw[style=dashed] (1,1) rectangle +(3.0,2.75);

\foreach \x in {0,1}
  \foreach \y in {0,1}  
  \shade[ball color=blue] (1.5*\x,1.5*\y) circle (0.25cm);

\node at (0.8,4.5) {(d)};
\end{tikzpicture}
\end{minipage}
\ \\ \ \\


